Finding Neurons in a Haystack: Case Studies with Sparse Probing

Despite rapid adoption and deployment of large language models (LLMs), the internal computations of these models remain opaque and poorly understood. In this work, we seek to understand how high-level human-interpretable features are represented within the internal neuron activations of LLMs. We train $k$-sparse linear classifiers (probes) on these internal activations to predict the presence of features in the input; by varying the value of $k$ we study the sparsity of learned representations and how this varies with model scale. With $k=1$, we localize individual neurons which are highly relevant for a particular feature, and perform a number of case studies to illustrate general properties of LLMs. In particular, we show that early layers make use of sparse combinations of neurons to represent many features in superposition, that middle layers have seemingly dedicated neurons to represent higher-level contextual features, and that increasing scale causes representational sparsity to increase on average, but there are multiple types of scaling dynamics. In all, we probe for over 100 unique features comprising 10 different categories in 7 different models spanning 70 million to 6.9 billion parameters.

==> old.tex <==


% In this work, we seek to understand how high-level human-interpretable features are represented within LLMs by training $k$-sparse linear classifiers (probes) on the internal neuron activations of LLMs to predict the presence of features in the input. By varying the value of $k$ we study the sparsity of learned representations and how this varies with model scale.
% More broadly, we show there exists lots of interpretable structure within LLMs that can and should be understood by humans.

% We show that early layers represent token-level features with significant compression by leveraging linear combinations of neurons that represent many features, and superposition, features that are usefully represented as , the first example of superposition in real models.

% In particular, we show that early layers make use of sparse combinations of neurons to represent many features in superposition

% In particular, we show that early layers represent many features with sparse combinations of neurons in superposition

% RS everyithing is a direction
% MLP things will be sparse in the privledged basis


%  We show that early layers represent token-level features with significant compression and interference and exhibit polysemanticity, neurons that represent many features, and superposition, features that are usefully represented as linear combinations of neurons, the first example of superposition in real models. We show that middle layers having seemingly monosemantic representations of contextual features, such as the language of text or programming language of code. We examine how sparsity of representations varies with model scale, and exhibit suggestive evidence of neuron splitting and quantization.

%  In particular, we show that early layers make use of sparse combinations of neurons to represent many features in superposition, that middle layers have seemingly dedicated neurons to represent higher-level contextual features, and that increasing scale causes new features to form and other features to split. More broadly, we show there exists lots of interpretable structure within LLMs that can and should be understood by humans.

% We show that early layers represent token-level features with significant compression and interference and exhibit polysemanticity, neurons that represent many features, and superposition, features that are usefully represented as linear combinations of neurons, the first example of superposition in real models.
% Despite rapid adoption and deployment of large language models (LLMs), the internal computations of these models remain opaque and poorly understood. In this work, we seek to understand how high-level human-interpretable features are represented within LLMs by training $k$-sparse classifiers (probes) on the internal neuron activations of LLMs to predict the presence of features in the input. By varying the value of $k$ we study the sparsity of learned representations and how this varies with model scale. With $k=1$, we localize individual neurons which are highly relevant for a particular feature, and perform a number of case studies to illustrate general properties of LLMs like monosemanticity, polysemanticity, superposition and neuron splitting.
% In all, we probe for over a 100 unique features comprising 11 different categories in 7 different models spanning 2 orders of magnitude in parameter count.

% Neural networks are frequently criticized for their inherent lack of interpretability. Modern large language models (LLMs) are hundreds of billions of parameters with dense high dimensional representations that lack any reason or incentive to be scrutable to humans. However, the same could be said of most natural phenomena, with a similar sense of daunting complexity faced by early scientists in emerging disciplines. Often progress is made most rapidly when applying a novel lens to view the relevant phenomena in a new light: the microscope in biology, telescope in astronomy, sequencer in genetics, fMRI in neuroscience. In this work, we strive to better understand modern language models by applying a discrete optimization lens \cite{bertsimas2019machine}. 

% Neural networks are frequently criticized for their inherent lack of interpretability. Modern large language models (LLMs) are hundreds of billions of parameters with dense high dimensional representations that lack any reason or incentive to be scrutable to humans. Many doubt whether these models ``think'' in a way that we can interpret at all. Yet many thriving fields today, such as cellular biology, genetics, or neuroscience, were similarly incomprehensible and daunting to early pioneers. We believe artificial neural networks can be interpreted---even reverse-engineered---but doing so requires a comparable amount of effort as interpreting biological ones. This is an extremely ambitious proposal, but given the potential risks and opportunities of LLMs \cite{bommasani2021opportunities,ngo2023alignment}, we deem it necessary.

% Neural networks are frequently criticized for their inherent lack of interpretability. Modern large language models (LLMs) are hundreds of billions of parameters with dense high dimensional representations learned via stochastic gradient descent (SGD) that lack any reason or incentive to be scrutable to humans. Yet, the same could be said of all life sciences studying the structures ``learned'' by natural selection, exhibiting similarly incomprehensible and daunting to early pioneers. We believe artificial neural networks can be interpreted---even reverse-engineered---but doing so requires a comparable amount of effort as interpreting biological ones: an \textit{artificial neuroscience}. This is an extremely ambitious proposal, but given the potential risks and opportunities of LLMs \cite{bommasani2021opportunities,ngo2023alignment}, we deem it necessary.


% As applied to language models, the basic principle is to train a classifier (a probe) on the internal representations of a network to predict a property of the input for which we have some external labels (e.g., the part-of-speech of the current token). Typically, a linear classifier is trained on all of the internal activations for each layer of a network. High classification performance of the probe is then evidence that the feature, or at least a close correlate, is represented at a specific layer in the network.


% The natural next question to ask is \textit{how} a feature is represented, and in particular, how sparse? On one hand, the literature contains many isolated examples of features  being represented by single neurons for a variety of tasks and architectures \cite{radford2017learning, bau2020units, olah2020zoom, goh2021multimodal, elhage2022solu}. However, given the complexity of natural language, there are many more features worth representing than there are neurons in a language model, incentivising the network to employ a form of compression to represent $m$ features in $n$ dimensions where $m \gg n$, termed \textit{superposition}. This necessarily manifests in individual neurons firing for multiple unrelated stimuli, a phenomena known as \textit{polysemanticity}. Such polysemantic neurons pose a challenge for interpreting and ultimately reverse-engineering neural networks as when representations are tangled \cite{elhage2022toy} it undermines our ability to study any component of a network in isolation.

% Recent work has begun to analyze how, why, and when neural networks perform this \textit{superposition} of features across dimensions in simplified settings \cite{elhage2022toy, scherlis2022polysemanticity, jermyn2022engineering}. This early work suggests that features are more likely to get a dedicated neuron the more important the feature is to the learning task or the more prevalent it occurs in the input. As features decrease in prevalence or importance, they become embedded in non-orthogonal subspaces with other features that rarely co-occur together. It then becomes the job of neurons in the feed forward layers to ``clean-up'' the interference between non-orthogonal features, and perform the relevant computation.
% - More narrative flow: naive hypothesis that neurons are interpretable; work observed polysemanticty and entanglement; picture is more complicated; maybe superposition where models trade off capacity and interference; we need richer tools to measure this and use sparse probing to investigating

% Motivated by results in these toy settings, in this work we attempt to study how these insights transfer to full-scale transformer-based generative pre-trained (GPT) language models by training sparse probing classifiers for a large number of features and levels of sparsity. We begin by comparing the performance of different feature selection methods in identifying relevant neurons, including moment methods, mutual information, $l_1$ regularization, and recent advances in optimal subset selection \cite{bertsimas2020sparse, bertsimas2021sparse}. Using these methods, we then demonstrate the relationship between model size and representational sparsity for a variety of human-interpretable features. Finally, guided by sparse probing, we conduct a series of more detailed case studies on specific neurons to elucidate a number of general observations about the representations of language models in addition to illustrating subtleties of applying and interpreting sparse probing results. In all, we probe for over a 100 unique features comprising 11 different categories in 7 different models spanning 2 orders of magnitude in parameter count (up to 6.9 billion) yielding the following insights:
% \begin{itemize}
%     \item Representational sparsity increases with model size, but there exists a countervailing force of neuron splitting.
%     \item Many early layer neurons are in superposition and therefore highly polysemantic, often firing for a diverse collection of $n$-grams. Moreover, based on weight statistics, we conclude that early layers employ more superposition than other parts of the network.
%     \item Higher-level contextual and linguistic features are often encoded by monosemantic neurons.
%     \item Sparse probing is an effective methodology to locate relevant neurons and study questions of superposition, but requires careful use and follow up analysis to draw rigorous conclusions.
% \end{itemize}



% we introduce \textit{sparse probing} and leverage recent advances in optimal sparse prediction \cite{bertsimas2020sparse, bertsimas2021sparse}. Probing is a standard technique used to study if and where a neural network represents a specific feature by training a simple classifier (a probe) on the internal activations of a model to predict a property of the input \cite{belinkov2022probing} (e.g., classifying the tense of a verb based on the activations of a particular layer). Sparse probing is the same, with the one additional restriction that the classifier can use at most $k$ neurons in its prediction. In addition to being well-suited for studying superposition (by systematically varying the value of $k$), sparse probing addresses a number of limitations identified in the probing literature.


% the full reality appears far more complex, especially for language models. In particular, most neurons in LLMs appear to be \textit{polysemantic}, activating for a large collection of seemingly unrelated stimuli \cite{elhage2022solu, mu2020compositional}. Such polysemantic neurons pose a challenge for interpreting and ultimately reverse-engineering neural networks because tangled representations undermine our ability to decompose the network into independently meaningful components \cite{elhage2022toy}.


% Recent work has proposed the \textit{superposition hypothesis} as a possible explanation for this phenomena \cite{elhage2022toy}. In particular, if there exists more features than neurons---likely given the complexity of natural language---then the model must employ a form of compression to embed $n$ features in $n > d$ dimensions, with polysemanticity being a logical consequence. However, this also causes loss-increasing ``interference'' between features. Results in toy models demonstrate that this tension manifests in a spectrum of representations: monosemantic for the most prevalent and important features with increasing levels of superposition for the long tail of rarer or less important features \cite{elhage2022toy, scherlis2022polysemanticity}. This can be formalized by measuring the sparsity of representations, that is, for each feature, how many neurons are being used to represent it? However, as these results are in toy models, it raises a number of additional questions: To what extent do these insights transfer to full scale language models? What kinds of features do or do not appear in superposition? At what scale? How do we reliably find and verify such (feature, neuron) pairs? What implications does all this have for interpretability? 
% For example, in a series of papers, \cite{olah2020zoom} demonstrates the presence of an interpretable circuit for recognizing cars, which consists of a hierarchy of neurons in successive layers that activate for increasingly abstract features like edges, curves, circles, wheels, and ultimately cars.

% \q{original para 2:}Neural networks are often conceptualized as being flexible ``feature extractors'' that learn to iteratively develop and refine suitable representations from raw inputs \cite{bengio2013representation,donahue2014decaf}. This begs the question: what features are being represented and how? Given models are parameterized as a series of dense matrix multiplications and elementwise nonlinearities, a natural hypothesis is that features are represented as linear directions in activation space \cite{elhage2022toy}, and are iteratively combined to synthesize increasingly abstract features using linear combinations of previously computed features \cite{olah2020zoom}. For example, in a series of papers, \cite{olah2020zoom} demonstrates the presence of an interpretable circuit for recognizing cars, which consists of a hierarchy of neurons in successive layers that activate for increasingly abstract features like edges, curves, circles, wheels, and ultimately cars.


% \q{original para 3:} Following this reasoning, one might hope there exists a 1:1 correspondence between features of the input and neurons in a network, making the core problem of interpretability simply constructing this mapping. While the literature contains many isolated examples of such \textit{monosemantic neurons} for a variety of tasks and architectures \cite{radford2017learning, bau2020units, olah2020zoom, goh2021multimodal, elhage2022solu}, the full reality appears far more complex, especially for language models. In particular, most neurons in LLMs appear to be \textit{polysemantic}, activating for a large collection of seemingly unrelated stimuli \cite{elhage2022solu, mu2020compositional}. Such polysemantic neurons pose a challenge for interpreting and ultimately reverse-engineering neural networks because tangled representations undermine our ability to decompose the network into independently meaningful components \cite{elhage2022toy}.


% We conclude by noting that, in another encouraging display of consilience, the phenomena of different regions of the model employing different coding strategies for different functions bears resemblance to the diverse coding strategies employed by biological neural networks. In the brain, various regions are specialized for different tasks and employ distinct coding strategies. For example, the primary visual cortex (V1) uses simple and complex cells for processing visual information \cite{hubel1962receptive}, while the hippocampus employs place cells and grid cells for spatial navigation \cite{o1971hippocampus, hafting2005microstructure}. Similarly, the olfactory system uses combinatorial coding to represent various odorants \cite{wilson1999combinatorial}. These diverse coding strategies reflect the specialized functions of different brain regions.

% different brain regions with different functional roles employ different coding strategies, analogous to how different layers with different functional roles appear to employ varying degrees of superposition. 

% In fact, it is possible to embed an arbitrary number of the mutually exclusive binary features in two dimensions, and perform a lossless recovery using essentially the first half of an MLP layer. The full construction is given in \td{superposition construction}, but the relevant fact is that it relies on having neurons with large weight norms combined with very negative biases to clean up interference. Motivated by this observation, we measure the product of the input weight norm and bias for each neuron in every layer and every model and record the median across layers. Figure~\ref{fig:norm_bias} illustrates the striking and consistent drop within the early layers (modulo layer 0 due to the parallel attention of Pythia models), in line with what our stylized theory would predict if early layers were most employing superposition to activate on every possible $n$-gram (the full distributions are available in Figure~\ref{fig:norm_bias_distribution}).


% \td{maybe cut and move to FAQ; binary encodings are bad geometrically} While our stylized reconstruction argument required an equal number of neurons and features, real models need to make do with far fewer. Consider a layer with neurons which fire for disjoint sets of size $k = m / n$ equally likely and mutually exclusive binary features (like $n$-grams; in other words, features are superimposed within a single neuron, as might be done with a naive finite approximation of our unit-circle embedding from before). While this layer can react to every feature, it remains ambiguous which of the $k$ features any activating neuron is reacting to. Far more effective would be to employ a binary encoding, requiring only $n = \log_2 m$ neurons, where each neuron encodes one bit of the feature identity.
% % \footnote{Of course this is also quite stylized. In particular, it is not just the job of a neurons to detect features (which need not be mutually exclusive or binary) but also to compute something meaningful}. 
% This manifests in half of the neurons (on average) firing for any particular feature. In practice, when we analyze the activation patterns of compound words, we indeed see many neurons in the \textit{same layer} react to the relevant bigram \texttt{XY} while not firing for \texttt{XZ} or \texttt{WY} (Figure~\ref{fig:sup_demo}). This amounts to a real demonstration of superposition of features across neurons.


% We conclude this case study by observing that many of the concepts and phenomena discussed so far have potential analogues in neuroscience. In particular, coding theory studies how neurons in the brain map to sensory stimulus. On one extreme, local coding theory posits the existence of ``monosemantic'' biological neurons which respond to a very specific stimulus (e.g., pictures of Jennifer Aniston \cite{quiroga2005invariant}). There also exists sparse coding theory and dense (or population) coding theory which suggest that a sparse (dense) number of neurons to represent information, potentially corresponding to increasing levels of polysemanticity in the brain. 
% We believe that creating further connections between biological and artificial neural networks is an especially fruitful line of research.


% Connections to neuroscience
% - coding theory (neuroscience and computer science)
% - different brain regions use different coding schemes
% - promising direction to create taxonomies 


Understanding how language models represent factual information is of substantial importance for making progress on hallucinations, bias, fairness, and alignment. Previous work has shown that there exist certain ``knowledge neurons'' responsible for factual recall, and that, by manipulating the weights or activations, it is possible to edit these facts \cite{dai2021knowledge, meng2022locating}. In this case study, we examine a few such knowledge neurons in more detail. We identify these factual neurons by sparse probing the activations on the tokens comprising the surname of notable people to predict properties like their gender or occupation.

Figure~\ref{fig:fact_main} illustrates a few specific examples of neurons which are strongly predictive of different factual properties of people. In general, we found that mid-layer neurons had the highest density of factual neurons, and that it made little difference performing max-aggregation over all tokens in the surname as opposed to just probing the last token of the subject surname---exactly in line with the results from \cite{meng2022locating}. However, because the probing dataset just contains the activations name tokens, our results do not distinguish between, for example, the \texttt{is\_politician} and \texttt{is\_political} features. To gain additional insight, we perform a vocabulary analysis, analyzing both the tokens which on average most excite a neuron and which tokens have output embeddings with highest cosine similarity to the neurons output weight. 

% \td{add fig and analysis; prediction: ice-hockey neurons fires on everything about ice hockey}.

Additionally, these neurons can be causally implicated in the recall of a fact by ablations. In particular, for a few-shot question-answer task\footnote{For example, for the \texttt{sex\_or\_gender} property we use 3-shot prompting of the form, "Arthur Sullivan has gender male. Abraham Lincoln has gender male. Winona Ryder has gender female. Kalki Koechlin has gender". Note, this is also important as a baseline establishing that a model ``knows'' a fact in the first place.}, we measure the difference in logit of the correct answer between a nominal model and a model with the implicated neuron set to zero for all tokens. We find that ablating individual neurons in large models has a small overall effect on the output logits and predictive capabilities of the model. This indicates that either there exists some sort of ensembling of neurons, some learned backup behaviour\cite{wang2022interpretability}, or that, rather than ``computing the fact,'' these neurons are performing contingent processing based on a fact computed earlier in the model (e.g., controlling the gender of a pronoun). 

% \td{fig + short analysis}

This case study illustrates two additional subtleties when determining the presence or absence of superposition. First, sparse probing does not distinguish between a feature in superposition and a coarse feature represented as the union of multiple monosemantic neurons representing features of greater granularity (e.g., \texttt{is\_athlete} = \texttt{is\_football\_player} + \texttt{is\_hockey\_player} ...). A reasonable first approximation however, is to analyze the cooccurence of activations. A feature in superposition must be represented by all neurons activating simultaneously, where for a coarse feature, we would expect exactly one neuron to fire for any input within the positive class. Second, sparse probing \textit{can} give a rough indication of whether a feature is in superposition by reasoning about the flatness of the sparsity curve. That is, if increasing $k$ does not yield increasing classification performance, it is less likely that a feature is in superposition.

% \td{add FAQ}.

% -Mechanisms of factual knowledge important for bias/fairness, hallucinations, high stakes, alignment (ELK)
% -Probing for facts about people

% -Results
% -Many neurons which do in fact code \td{Vocab analysis to distinguish basketball-player neuron from basketball neuron}; limitation of probing
% - Similarity to Bau results
% - Nevertheless, we can causally link these neurons to predictions \td{ablations}

% Subtleties
% - Ambiguity between feature being represented in superposition and composite feature (can look at activation cooccurence)
% - How to distinguish a discriminating neuron on the dataset from a being in superposition with other neurons (again cooccurence probably sensible; look at sparsity curves)


% In this case study we examine \textit{factual neurons}--neurons associated with information about real-world entities such as the location of cities. Though a wide range of such neurons may exist, we restrict our search to properties of people, both living and historical. Specifically, we apply sparse probing to see if the model can recall their gender, occupation, and whether or not they are alive from their name. We subdivide each of these properties into binary features such as \texttt{gender\_is\_male} or \texttt{occupation\_is\_politician}. 

% We know that the models must have some internal representation for these features as they can reliably generate the correct class when prompted \td{(subjectively true but run this experiment)}, but the structure of these representations is not well understood. While sparse probing alone can not be used to establish a causal link between the activations of a set of neurons and a model's outputs, it can provide evidence that the model has some internal representation for a feature and additionally where in the model that representation is most coherent. 

% To identify these neurons using sparse probing we run sequences containing names through the model and probe the activations of the tokens for the names using the known values for the property features. Specifically, we probe the maximum over the activations for the tokens of the surname in an attempt to limit the impact of correlations between first names and the selected property (e.g. gender can often be inferred from a person's first name) and hope that the selected neurons instead are capturing factual knowledge about the person. We draw sequences from the test set of The Pile and property information from Wikidata\footnote{\url{https://www.wikidata.org}}.

% A selection of the neurons we found in the Pythia-6.9B model is presented in Figure \td{5}. For each neuron we plot its activation value for each of the classes in the relevant property. We find that the activations of single neurons contain enough information to discriminate between people of according to the listed properties. For occupation, we find that the neurons for predicting type of athlete within the subset of all athletes are generally better than those for predicting more general occupations. This suggests that feature granularity (i.e. how far to subdivide features) has an effect on the abundance of factual neurons and that certain factual features may be represented through multiple, monosemantic neurons representing subcategorizations of the original feature.

% \td{now that i'm writing this i'm realizing that we should probably have looked for a grouped athlete neuron but alas}


% \td{not sure what all we want to say here}



% Notes from Wes

% \cite{dai2021knowledge, meng2022locating} 
% \begin{itemize}
%     \item Main figure: Neurons firing for gender, profession, dead or alive of people. Comparison against zero-shot/few-shot baseline with and without ablation. Potentially also sparsity curves + top average vocab
%     \item Probing limitation: does not distinguish between \texttt{politician} neuron and \texttt{politics} neuron, i.e., a neuron which fires on all tokens related politics, of which politicians are only a subset.
% \end{itemize}

% People are interested in control and being surgical about making modifications, cite othello, surgically make modifications. Important and relevatn bc models are filled with these biases, promise of mech interp which motivates;
% ablations
% probing cannot causally link. 

% Can try to verify not superimposed by looking at sparsity curves.

% Superposition vesus composite features can be difficult to disentangle (eg. is athelete being sum of individual athletic activities; can get some idea based on whether the neurons always fire together or not)


% \subsection{Syntactic Neurons}
% \td{TODO; probably cut for general exam draft}
% \begin{itemize}
%     \item Main figure: compilation of sparse linguistic features. Active/passive verb, end of sentence (which increases prob of capital next tokens and decreases lowercase). Weird large activation first sentence neurons. Maybe: position, other EWT features
%     \item Perhaps something to illustrate granulaity mismatch (maybe proper noun).
% \end{itemize}
% % \subsection{Prediction Neurons}
% % TODO. Candidates: calibration, top class probability, next token bigram/linguistic feature


% Rather than just localize a feature to a direction in a layer, we attempt to identify a single neuron or a sparse subset of neurons which fire if (and ideally only if) the feature is present in the input. This can be accomplished by training a $k$-sparse probe, a linear classifier with at most $k$ non-zero coefficients. The problem becomes, of the up to tens of thousands of neurons per layer, which subset of $k$ neurons are most predictive?

While this is an $\mathcal{NP}$-hard combinatorial optimization problem, there exists a number of fast heuristics and tractable optimal algorithms \cite{tillmann2021cardinality}. In particular, we will compare the performance of a logistic regression trained using the $k$ neurons selected with the following approaches (see the Appendix for a formal description of each approach). \td{rewrite as paragraph}
% \td{citations and formal descriptions in appendix; Telescoping versions.}
% In Section~\ref{sec:results} we compare the classification performance of
\begin{enumerate}
    \item Max mean difference (MMD): independently for each neuron, compute the maximum absolute difference in the activation class means and select the top $k$ neurons\cite{antverg2021pitfalls}.
    % $\sum_{jt: z_{jt} = 1} a_{jt}^{(\ell)} - \sum_{jt: z_{jt} = -1} a_{jt}^{(\ell)}$
    \item Mutual information (MI): independently for each neuron, compute the mutual information with the class label and select the top $k$ neurons \cite{ross2014mutual,voita2020information,pimentel2020information}.
    \item $l_1$ regularized (L1): choose the $k$ neurons with largest coefficient magnitudes after training a dense probe with $l_1$ regularization \cite{dalvi2019one}.
    \item F-statistic (FS): choose the $k$ neurons with the largest F-statistic of a one way ANOVA between the two class distributions.
    \item Optimal sparse probing (OSP): choose the $k$ neurons selected by an optimal cardinality constrained classifier \cite{bertsimas2021sparse}.
\end{enumerate}
To our knowledge, FS and OSP are novel in the context of probing. Additionally, note that while we focus on classification, all of these methods have a straightforward generalization to continuous targets.
